Schr\"odinger cat states of a 16-microgram mechanical oscillator

The superposition principle is one of the most fundamental principles of quantum mechanics. According to the Schr\"odinger equation, a physical system can be in any linear combination of its possible states. While the validity of this principle is routinely validated for microscopic systems, it is still unclear why we do not observe macroscopic objects to be in superpositions of states that can be distinguished by some classical property. Here we demonstrate the preparation of a mechanical resonator with an effective mass of 16.2 micrograms in Schr\"odinger cat states of motion, where the constituent atoms are in a superposition of oscillating with two opposite phases. We show control over the size and phase of the superposition and investigate the decoherence dynamics of these states. Apart from shedding light at the boundary between the quantum and the classical world, our results are of interest for quantum technologies, as they pave the way towards continuous-variable quantum information processing and quantum metrology with mechanical resonators.

==> Cat state in cQAD Arxiv/commented_text.tex <==
% The absurd conclusion of this hypothetical scenario seems to indicate that our current understanding of quantum mechanics is incomplete.

%The bottom chip holds the single junction aluminum qubit which we design for operation in the transmon regime \mb{citation}. The sapphire top chip is used as the HBAR substrate. Coupling between qubit and HBAR is induced through a dome shaped layer of piezoelectric Aluminum Nitride. The piezoelectric acts as a transducer between the electric field of the qubit and the strain field of the HBAR, while the dome shape functions as a curved phononic mirror, confining the phononic mode volume in transverse direction. The phonon modes hosted by this resonator geometry are characterized by two transversal mode numbers $p,l$ and one longitudinal mode number $m$, where the transverse modes are described by Laguerre-Gaussian basis functions and longitudinal modes by sinusoidals respectively. We add a circular antenna below the piezoelectric transducer to shape the transverse qubit electric field into a Gaussian, optimizing for coupling to the fundamental transverse mode with $p=l=0$. 

%With a qubit frequency of around $6\,$GHz, the longitudinal mode we select has a high overtone $m\approx 450$.
%Operating the device in a commercial dilution refrigerator at temperatures around $10\,$mK, the phonon mode we select is operated in the ground state. We then induce resonant energy exchange between qubit and phonon mode by tuning the qubit on resonance for a suitable amount of time. 

%### OLD VERSION: If we consider a coherent state in the acoustic mode, we  find a direct correspondence between the amplitude $\alpha$ of the displaced vacuum state in phase space and the physical oscillation amplitude in longitudinal direction of the atoms in the HBAR mode volume, proportional to $\alpha$ (see supplementary \ref{si:effective mass}). A sketch of the lattice displacement can be seen in the inset of Fig.~\ref{fig1}a). Here the pink and blue atom cores illustrate a crosscut of two neighboring atomic crystal layers, showing a snapshot in time of two longitudinal displacements of opposite amplitudes.

% Continue with half revival time here.
% Considering the time evolution of the full system state without tracing out the phonon subsystem, if the qubit initialized to $\ket{e}$ state, the resonance interaction lead to entanglement between the qubit and phonon state at $t_{\textit{collapse}}$. As a measure for entanglement between qubit and phonon state, we can regard the qubit purity defined as  $\gamma(t)=\text{Tr}\left(\rho_\text{qb}(t)^2\right)$, where $\rho_\text{qb}(t)$ is the reduced density matrix of the qubit subsystem. Monitoring $\gamma(t)$, directly indicates the degree of entanglement in the system during the resonant interaction. Following the trajectory of $\gamma(t)$ in Fig.\ref{fig1}b, the dephasing of Rabi-oscillations coincides with a minimum at $t_{\textit{collapse}}$, indicating a maximally entangled state. 

% Going back to the language of superpositions between out of phase lattice oscillations in the HBAR substrate, we can assign a maximal spatial separation between atoms being part of the created Schr\"odinger's cat state.


% Numerical values for the effective displacements can be found in \ref{si:effective mass}. 
%We can therefor confirm the creation of a coherent superposition between two atomic oscillation states which show a maximal physical distance of $2x^{\text{rms}}_\text{eff}= XXX$ with an effective oscillating mass of $XXX$. 

%As described in previous works\cite{vonLupke22}, our system consists of a plano-convex HBAR fabricated using piezoelectric aluminum nitride (AlN) on a sapphire substrate and a superconducting qubit on a separate sapphire chip, which are then combined into a device called the $\hbar$BAR. The AlN couples the electric field of the qubit with the strain field of the HBAR modes, resulting in a Jaynes-Cummings (JC) type interaction between the two quantum systems.
%Here, we use a single-junction, non-flux tunable transmon qubit and house the $\hbar$BAR inside a superconducting Al cavity. previous devices. All frequency tuning is performed by applying microwave drives to Stark shift the qubit instead of applying an external magnetic field\cite{ChuScience2017}. With our current system parameters and electronic hardware, we are able to Stark shift qubit frequency more than 50 MHz, which enables us to manipulate multiple phonon modes. 
%In order to prepare a cat state of phonons, we make use of the coherent resonant interaction between the acoustic mode and the qubit \cite{BuzekPRA92}. The latter provides the nonlinearity necessary for the preparation of non-Gaussian states of the oscillator. 

%%%%%%%%%%%  Below: Previously Matteo's description of Fig2. Now merged %%%%%%%%%%%         into Fig.1b) explanation. Here we want to discuss 
%%%%%%%%%%%         the experiment only
%For a qubit initially in the excited state, and an phonon mode in the vacuum state, Eq.~\eqref{eq:HJC} results in vacuum Rabi oscillations between the qubit and phonon population~\cite{Chu2018}.
%On the other hand, if the phonon mode is in a coherent state $\ket{\alpha}$, the time evolution of the resonant interaction is considerably more complex \cite{Cummings65,EberlyPRL80}. In particular, it is known that the qubit population oscillates showing periodic collapse and revivals. Intuitively, the collapse occurs because the JC interaction's frequency depends on the number of excitations in the bosonic mode, which for a coherent state is given by a Poissonian distribution. %This oscillation undergoes a collapse due to the dispersion of the Rabi frequencies associated to different photon numbers.
%Therefore, oscillations with different frequencies rapidly dephase, showing a decay of the qubit oscillation amplitude as \cite{Rempe87} $\text{exp}(-(t/t_{\textit{collapse}})^2)$, where $t_{\textit{collapse}}=\sqrt{2}/g$ is the collapse time.
%If the phonon field were classical, the distribution of oscillation frequencies would just result in a decaying signal. However, the phonon energy quantization results in a discrete oscillation frequency spectrum, resulting in oscillations that rephase in finite time. For $\alpha \gg 1$ this revival occurs at $t_R = 2 \pi \alpha/g$ \cite{EberlyPRL80}.

%%%%%%%%%% Matteo's version of Fig2
%Fig.~\ref{fig2}a shows the experimental sequence we use to observe such collapse and revival in our system. First, we prepare the phonon mode in a coherent state by sending a resonant drive pulse of amplitude $A$. After the phonon drive, we cool down the qubit with an ancilla phonon mode to eliminate the effect of the phonon drive on the qubit. Then, we initialize the qubit state in the excited state with a Gaussian shaped $\pi$ pulse. Afterwards, we let then the two system resonantly interact for a time $t$, after which the qubit state is measured. The results are shown in Fig.~\ref{fig2}b for $A=0.35$ (corresponding to $\alpha = 1.75$). As expected, we observe a collapse of the ocillation amplitude after a time $t_{\textit{collapse}}\approx\unit{...}{\mu s}$, and a revival at $t_R\approx\unit{...}{\mu s}$. These effects are genuine quantum features, originating from the phonon energy quantization.
%The observation of revivals in the oscillation also reveals a coherent energy exchange in the qubit-phonon system \cite{MeunierPRL05}. Moreover, it is predicted that at time $t_R/2$ the state of the system resembles a Schr\"odinger's cat state\cite{BuzekPRA92}.

%The first row in Fig.~\ref{fig2}c shows snapshots of the collapse-revival dynamics, obtained by performing Wigner tomography of the phonon mode at different evolution times, using the tools demonstrated in Ref.~\cite{vonLupke22}.
%Here, we normalize the measured Wigner value based on the dispersive parity measurement result of phonon Fock $\ket{0}$ state.
%We normalize the axes of the Wigner functions by measuring the phonon Fock state distribution of coherent states created with different drive amplitudes as demonstrated for example in \cite{Chu2018}. 
%As expected, the initial coherent state (Fig.~\ref{fig2}c upper left), evolves into a cat state at $t_C=2.9\,{\mu s}$ (Fig.~\ref{fig2}c upper middle), and then refocuses into a state that for large $\alpha$ resembles a coherent state ( Fig.~\ref{fig2}c upper right). For comparison, we plot in the second row of Fig.~\ref{fig2}c the exact state evolution we expect from $H_{JC}$  for the interaction time as the corresponding measurement ones (see supp), showing good agreement with the data. 

% Following the linear dependence between $t_R/2$ and $\alpha$, for the measured phonon states displayed in the top row of Fig.~\ref{fig3}a), the smaller initial $\alpha$ result in interaction times $t_C = 2.40\,\mu$s and $2.70\,\mu$s. 

% , as well as a finite background offset of the parity values \cite{vonLupke22}.

%%The extracted state sizes $D$ of the ideal fits, the state sizes $\alpha_\text{fit}$ from the anlytical fits together with the associated fidelities to the reconstructed states are summarized in Fig.\ref{fig3}b. Noting that the interaction times $t_C$ for $A=0.25$ and $A=0.30$ are closer to $t_R/2= 2.42\,\mu$s and $2.90\,\mu$s, when compared to the deviation between $t_C$ and $t_R/2$ for the state with $A=0.35$, we can explain the similar values of $D$ and $\alpha_\text{fit}$ in case of $A=0.25$ and $A=0.30$. Since for these two states, the coherent components are more symmetric around the fringes when compared to the $A=0.35$ state from Fig.\ref{fig2}c, hence fitting to the ideal state gives a larger separation between the coherent state components $\alpha_1$ and $\alpha_2$. Again we accommodate the overall lower fidelities of the ideal states, to the analytical expression \eqref{eq:sup_exactState} only resembling and ideal Schr\"odinger's cat state in the limit $\alpha\rightarrow\infty$ (compare Supplementary A).


% The phase of a cat state is given by the parameter $\vartheta$ in eq.\eqref{eq: ideal_cat}. In the case of $\alpha_1 = -\alpha_2$, $\vartheta = 0$ ($\pi$) corresponds to an even (odd) parity state. 
% % Controlling the phase of the created Schr\"odinger's cat state allows to encode a qubit state in either the even or odd parity subspaces of the bosonic mode's Hilbertspace, a promising method in bosonic error correction codes\cite{Ofek2016}. Considering the Wigner function of Schr\"odinger's cat states, the fringes roll when changing $\vartheta$, where different superposition state shows different interference pattern.  
% To also obtain phase control over the cat states in our system, we vary the initial qubit state across the six cardinal points ($\ket{\pm X}, \ket{\pm Y}, \ket{\pm Z}$ of the Bloch sphere. 
% Since qubit operations are performed far detuned from the selected phonon mode, the qubit state acquires a relative phase in the phonon rotating frame. This results in a phase offset for the rotation axis of the qubit pulse required to reach the cardinal points listed above.
% %We compensate this phase offset by measuring collapse and revivals with the qubit initially prepared in a superposition $\ket{+Z}+e^{i\varphi}\ket{-Z}$, sweeping the phase of the rotation axis $\varphi$. We then pick the phase offset corresponding to the $\ket{+X}$ state, by selecting the one $\varphi$ that does not show oscillations of the qubit population (see supplementary Fig.\ref{fig:suppFig_cnr}). 
% After calibrating the phase offset (see supplementary \ref{Sup A.1}), we perform Wigner tomography on the phonon state with $A=0.30$ at $t_C=2.70\,\mu$s and the qubit initially in $\ket{\pm X}$, resulting in the first column of Fig.\ref{fig3}c. We observe a distorted coherent state located on the upper (lower) half of phase space for the qubit initially in $\ket{+X}$ ($\ket{-X}$), where the separation in phase space is expected from the opposite rotation direction between the two initial qubit states (compare Fig.\ref{fig1}c). As explained earlier, an initial qubit state $\ket{\pm X}$ approximately results in an eigenstate of \eqref{eq:HJC}. We can attribute the state distortions to a finite degree of entanglement during the resonant interaction. 

% Moving to the cardinal points $\ket{\pm Y}=\ket{Z}\pm i\ket{-Z}$, the second column in Fig.\ref{fig3}c shows Schr\"odinger's cat states with opposite phase at $t_C$, revealed by the interference fringes flipping sign between $\ket{+Y}$ and $\ket{-Y}$. We deduce that the phase information of the qubit initial state has fully mapped onto the phonon state at $t_C$. Measurements for the final two cardinal points $\ket{\pm Z}$ are shown in the third column of Fig.\ref{fig3}c. The different shapes between the $\ket{\pm Z}$ states can be understood by noting that for $\ket{+Z}$ the qubit initially is in its ground state, whereas for $\ket{-Z}$ it is prepared in the excited state, contributing one energy quantum $\hbar\omega_{\text{ph}}$ to the total energy of the system when on resonance with the phonon mode. With an average population of $\alpha^2\approx2.3$ of the initial coherent state, the energy contribution of the qubit to the total energy in the system is considerable, leading to the less pronounced fringes. Still the same flipping of parity in the fringes as also observed between $\ket{\pm Z}$ are clearly visible, indicating the qubit rotation angle has mapped onto the phonon state phase at $t_C$.   

% In summary, we conclude the possibility of preparing states that have a fidelity $\geq 65\%$ compared to ideal Schr\"odinger's cat states, with an $\alpha_{\text{fit}}=1.51$, as well as full phase control over the created states by choosing the appropriate initial qubit state.


%%%% Uwe's version
%After showing how we create an approximate cat state in a phonon mode, we move on to demonstrate how we control the amplitude and the phase of such a state. 
%We vary the amplitude $A$ of the initial phonon displacement drive (see Figure \ref{fig2}a) to change the amplitude of the coherent state thus created. 
%As depicted in Figure \ref{fig2} the coherent state evolves into an approximate cat state during an interaction time $t_\mr{cat}\approx t_R/2=\pi\alpha/g$. 
%Note that this time depends on the size $\alpha$ of the coherent state so it has to be adjusted for different cat sizes. 
%The cat state now has an amplitude $\alpha_\mr{cat}$ proportional to the initial drive amplitude $A$. 

%In addition to the cat state depicted in Figure \ref{fig2}c, we show two more cat states with displacement drive amplitudes $A=0.25$ and $A=0.30$ in Figure \ref{fig3}a. 
%As in Figure \ref{fig2}c, we fit the analytical states resulting from a decay-free evolution of the initial coherent state to the data. 
% From the fit we extract the cat sizes $\alpha_\mr{fit}$, displayed in the corner of the Wigner functions of the analytical states in Figure \ref{fig3}a.  
% We also fit an ideal cat state $\ket{\psi_\mr{ideal}}=\ket{\alpha_1}+e^{i\vartheta}\ket{\alpha_2}$ and find the resulting ideal cat size $\alpha_\mr{ideal}=|\alpha_1-\alpha_2|/2$ of the ideal cat state with the highest fidelity to the measured states. 
% We display both the sizes of the best-fit approximate \textcolor{red}{analytical?} and ideal cat states in Figure \ref{fig3}b over the amplitude $A$ of the displacement drive used to create them. 
% We observe a linear relationship between the displacement amplitude and the cat size up to $\alpha_\mr{fit}=1.61$ with fidelities between the density matrix reconstructed from the data and the analytical state around 80\%, as well as fidelities of 65\% and more between the created states and ideal cat states. 

% Now that we have shown how we control the size of the approximate cat states we create, we move to explain how we can control their phase. 
% In an ideal cat state this phase corresponds to the parameter $\vartheta$ in $\ket{\psi_\mr{ideal}}$. 
% In the state created by the evolution under a resonant Jaynes-Cummings interaction between a coherent state in the phonon mode and the qubit, the initial qubit state maps onto the phonon state at the time $t_{cat}$ as follows. 
% Writing the initial qubit state as $\ket{\psi_\mr{qb}(0)} = c_+\ket{+x}+c_{-}e^{i\vartheta}\ket{-x}$, with $\ket{\pm x}=(\ket{g}\pm\ket{e})/\sqrt(2)$, the phase $\vartheta$ is the angle between the complex amplitudes of the $\ket{\pm x}$ states. 
% Over the time $t=t_\mr{cat}$ the phonon state then evolves into a superposition $\ket{\psi_\mr{JC}(t_\mr{cat}}=c_+\ket{\psi_{+}}+c_{-}e^{i\vartheta}\ket{\psi_{-}}$ of two approximately coherent states $\ket{\psi_{\pm}}$. 
% For the detailed derivation, see the Supplementary Information, section \ref{si:state_evolution}. 
% The phase $\vartheta$ and the amplitudes $c_{\pm}$ of this superposition are those of the initial qubit state. 
% In Figure \ref{fig3}c, we show Wigner functions of $\ket{\psi_\mr{JC}(t_\mr{cat})}$ for different initial qubit states, indicated by the label in the top right corner of each plot. 
% When the qubit starts out in $\ket{\pm x}$ (Figure \ref{fig3}c, we observe two misshapen, elongated coherent states, sometimes colloquially referred to as \textit{bananas}. 
% As explained in the Supplementary Information, these states $\ket{\psi_{\pm}}$ approximate displaced coherent states with opposite amplitudes for sufficiently large initial displacements $\alpha$ of the phonon mode. 
% When the qubit starts out in an equal superposition of $\ket{\pm x}$, such as $\ket{\pm y}$ (Figure \ref{fig3}d) or $\ket{\pm z}$ (Figure \ref{fig3}e), the phonon state at $t_\mr{cat}$ is the superposition of the two bananas measured for $\ket{\pm x}$. 
% The position of the fringes is ideally determined by the phase of $\ket{\psi_\mr{qb}(0)}$, which can we observe in Figure \ref{fig3}d and e, noting that the position of the phases for $\ket{\pm y}$ and $\ket{\pm z}$ switches between blue and red. 
% Due to the finite average phonon number $\bar{n}$ in the coherent state the position of the fringes in our experiment differs slightly from the theoretical value corresponding to a $\pi/2$ phase difference between $\ket{\pm y}$ and $\ket{\pm z}$ . 
% The average phonon number for a displacement amplitude of $A=0.35$ is between two and three. Therefore, the energy difference between $\ket{\pm y}$ and $\ket{\pm z}$ changes the effective $\alpha_\mr{fit}$ and in consequence the correct $t_\mr{cat}$. 
% A changing $t_\mr{cat}$ leads to a roll-off of the measured $\vartheta$, because of the detuning between the rotating frame of the qubit drive (which is at the frequency of the qubit rest point) and that of the
% phonon mode. 

% \vspace{10mm}
% \textcolor{blue}{Matteo's version:\\}
% In the following, we demonstrate the control over amplitude and phase of the cat states we can prepare. To generate cat states with different mean phonon number we change the driving pulse amplitude $A$, and adjust the resonant evolution time accordingly. 
% In order to benchmark the generated cat states, we implement a maximum-likelihood reconstruction of the system's state $\rho$ from the collected parity measurements \cite{Chou2018}, and then compute the fidelity against a target state $\sigma$ as $F=\text{Tr}\left[\sqrt{\sqrt{\rho}\sigma\sqrt{\rho}}\right]$. As a first target state, we consider the analytical state resulting from evolving a coherent state $\alpha_a$ according to $H_{JC}$, see Supp Info. As a second target state, we consider the ideal cat state $\Psi_1 = \ket{\alpha_1} + e^{i\vartheta} \ket{\alpha_2}$, having amplitude $\alpha_i=\vert\alpha_1-\alpha_2\vert^2/2$. \mf{Maybe different name for the size? Like Haroche's $D$?}

% In Fig.\ref{fig3}a we show the measured Wigner functions of cat states prepared with two different values for $A$, together with the best matching analytical state resulting from evolving a coherent state $\ket{\alpha_1}$ with $H_{JC}$. These amplitudes $\alpha_1$, together with the amplitudes $\alpha_2$ of the best matching ideal cat states and with the associated fidelities, are summarized in Fig.\ref{fig3}b. We conclude the possibility of preparing states that have a fidelity $\geq 65\%$ compared to ideal cat states.

% Apart from the amplitude, it is of interest to control also the phase of the cat state, which is associated to the position and parity of the Wigner's interference fringes. In the limit of large $\alpha$ this phase can be fully controlled by the phase of the initial qubit state. In fact, one can observe collapse-revival dynamics for any initial qubit state on the $yz$-plane, resulting at $t_C$ in cat states with different phases (cite supp). On the other hand, preparing the initial qubit state along the $\pm x$ direction does not give any evolution to the oscillator's coherent state, as these are quasi-eigenstates of $H_{JC}$ \cite{GeaPRL90}.

% We demonstrate these ideas experimentally, by initializing the qubit's state along direction $\vec{v}\in\{\pm x, \pm y, \pm z \}$ before letting it interact resonantly for a time $t=...$ with the phonon mode prepared with $A=0.035$. The results are shown in Fig.\ref{fig3}c, where we can see the phonon mode to stay similar to a coherent state for $\vec{v} = \pm x$, while it evolves to cat states with different phases for $\vec{v} = \pm y,\pm z$. This measurement gives also an intuitive understanding of the dynamics resulting into cat states: an arbitrary qubit state can be seen as a superposition of $x$ eigenstates, and thus the evolution of the field as a superposition of evolutions of counter-rotating coherent states.

% \mf{Mention that the ability of preparing cat states with arbitrary phase is of interest for bosonic encoding of quantum information [Kerr cat qubit, ..].}



On the other hand, a coherent state should have a characteristic decay time $2T_1^{\text{ph}}$ to vacuum.



In the top row of Fig.~\ref{fig4}a, we show snapshots of the largest cat state with $A=0.35$ and $\alpha_\text{fit}=1.61$ at three different wait times $\tau=1, 5,$ and $50\,\mu$s, together with the reconstructed states in the row below. Note the fast decay of negative parity values after $5\,\mu$s compared to the slower decay speed of the classical state components towards the vacuum state. To quantify the characteristic timescale for the disappearance of quantum features, we make use of the time dependent negativity defined as $\delta(t) \equiv \int d^2\beta\,\vert W(\beta,\alpha, t)\vert - W(\beta,\alpha, t)$. Here, $W(\beta,\alpha, t)$ is the Wigner function of the cat state of size $\alpha$ at time $t$, and the integration is over all phase space, parametrized by the complex displacement amplitude $\beta$. Since $\delta(t)$ represents an integration over all negative values of $W(\beta, \alpha, t)$, it can be considered a measure for non-classicality of the state\cite{Kenfack04}. As shown in supplementary \ref{si:cat_decoherence}, in the limit of large $\alpha$,  $\delta(\tau)$ decays with a time constant $\tau_\text{cat}=T_1^{\text{ph}}/(2\alpha^2)$, while a coherent state should have a characteristic decay time $2T_1^{\text{ph}}$ to vacuum, explaining the different decay times of the aforementioned features in Fig.\ref{fig4}a.


We experimentally extract the timescales of negativity decay for cat states with four different initial displacement amplitudes $A$. Due to fluctuations of the qubit frequency during the dispersive interaction, we observe fluctuations in the background value of the measured Wigner functions \cite{vonLupke22}. We mitigate the contribution of these variations to the computed negativity by manually selecting an integration window in phase space enclosing only the interference fringes in the reconstructed state, where negative features of the Wigner function are expected to appear. We then calculated the negativity within this window using the measured Wigner function, which are together with the corresponding fits to an exponential decay model are presented in Fig.\ref{fig4}b.  The fitted negativity decay constants for all four cat state sizes are shown in Fig.\ref{fig4}c.
Apart from the smallest state size, we observe the decay times monotonically decreasing with $A$. This trend is confirmed by looking at the extracted decay times obtained from a full Master equation simulation of the state decay with the reconstructions of the measured states set as the intial state in the simulation. An explanation for the low decay time of the smallest cat state is given in supplementary Fig.\ref{fig:suppFigCatPhaseDecays}. Simulating the decay of an ideal Schr\"odinger cat state (see eq.\eqref{eq: ideal_cat} with different $\vartheta$ and $\alpha_1 =-\alpha_2$, it can be seen that for state sizes $\alpha_1\lesssim1.5$, the decay rate becomes dependent on $\vartheta$. For $\vartheta$ small, this results in a drop in the decay time below $\alpha_1\lesssim 1.1$ coinciding with the decay time we observe in the reconstructed negativity of the smallest state.    

% \vspace{10mm}
% \textcolor{blue}{Matteo's version:\\}
% Superposition states are non-classical states that are notoriously prone to dec
herence. In order to investigate the quantum to classical transition of such states, we let the states we prepare evolve freely for some time $t$ before performing Wigner tomography. Then, we compute the negativity of the reconstructed Wigner function at time $t$ as $\delta(t) \equiv \int d^2\alpha \Big( \vert W(\alpha)\vert - W(\alpha) \Big)$, which is an indicator of nonclassicality~\cite{Kenfack04}. Computing the negativity at different times allows us to observe the disappearence of quantum coherences, and to extract the associated timescale.

% In Fig.~\ref{fig4}a we show a selection of snapshots for the decay of a cat state prepared with $A=XXX$. Similar measurements have been taken for the cat states with $A=XXX$. Selecting a phase-space region enclosing the fringes we are able to compute reliably $\delta(t)$, without being much affected by noise and imperfections in the background. The values we obtain are shown in Fig.~\ref{fig4}b, together with an exponential fit of the data. The decaying rates thus obtained are summarized in Fig.~\ref{fig4}c, together with theoretical and simulated predictions. 


% [drafted:] In Ref.~\cite{BrunePRA92,DelegliseNat08} it was investigated the decoherence of photon cat states under cavity losses at rate ($1/T_1$). It was found both theoretically and experimentally that off-diagonal elements decay for small times as $T_1/(2 \alpha^2)$ \mf{Here it would be beneficial to use a cat size parameter, rather than alpha.} We note that the same decay time is observed for the negativity of cat states of size $\alpha\gtrsim 2$ (see Supp Info). As our states are smaller than this, we perform a numerical simulation to predict their lifetime. The results are shown in Fig.~\eqref{fig4}c, and show good agreement between theory and simulation. 



% We measured Wigner functions of the generated cat state by the dispersive phonon parity measurement technique. The largest size of the generated cat state is $\alpha=1.51$, with a measured fidelity of $F\approx65\%$. We investigated the phase of generated cat state by initializing the qubit with different phase in the cat state generation sequence. 


% Generation the superposition of coherent states in macroscopic mechanical system is not only interesting in investigating the fundamental physics, such as collapse model of the macroscopic objects and the boundary between the classic and the quantum, but also useful ingredients for quantum information processing, such as quantum error correction and quantum metrology. For example, cat state in bosonic coding has been proposed and generated in cQED system, and $\hbar$BAR systems even have extra advantage of doing this, since the FSR of $\hbar$BARs is small and more phonon modes are available. In combination of the dispersive measurement of the phonon parity, error correction can be implemented in the cat state. Cat state has also been proposed for quantum metrology due to the high Fisher information at the fringe region. As a mechanical system, $\hbar$BAR can also be used for quantum-enhanced frequency or force sensing. For both investigating the fundamental physics and quantum information processing, requirements on qubit phonon coupling strength and sample coherence are similar, which implies better fabrication technique and device design is needed.


% We performed the Wigner tomography of these phonon states by using the displaced parity measurement procedure described in [parity paper]. 


% Each reconstructed phonon state $\rho_{r}$ was optimized for with Maximum Likelihood Estimation (MLE) fits to these measured Wigner functions, as described in Schoelkopf 2018: By imposing non-negative eigenvalues, Hermiticity and unit trace, we constrain the fit to only physical density matrices $\rho$. Each measured Wigner function is a set of measurement outcomes. Every $\rho$ will have an expectation value corresponding to each of these outcome. To find the MLE state $\rho_r$, we minimize the residual sum of squares over all measurements. The resulting optimization is a convex problem that can be efficiently solved as a constrained semi-definite programming problem.
% (Section S6B of https://arxiv.org/pdf/1801.05283.pdf)

% \textcolor{magenta}{Here we need to talk about the rescaling. For the reconstruction we can just cite previous work.} 

% Experimental imperfections and noise can give the measured Wigner functions artificially-offset features in the background. Simply carrying out the integral in Eq.~\eqref{eq:supp_WNegDef} over the full Wigner function phase space would therefore give an additionally noisy negativity estimate. To account for this background problem, we limit the integral to a sub-region of the phase space--the smallest sized window that fully encloses the negative fringes of each cat state. Using this method, we do not include any unphysical negative features present in the Wigner function, outside of the cat state, in our analysis of the negativity decay. Since we specify the windows to fully enclose all negative fringes of the cat state, performing the integral in Eq.~\eqref{eq:supp_WNegDef} only over the sub-region gives the same result as integrating over the full region (in the case of an ideal cat state with a perfect background). 

% To simulate the negativity decay of these states...


% \begin{figure}
% \centering
% \includegraphics[width=10cm]{figures/suppFigNegTest.pdf}
% \caption{\textbf{Cat decoherence rate from negativity.}
% Comparison between the cat decoherence rate obtained from a numerical computation of the Wigner negativity decay rate, and the rate $\tau_\text{cat} = T_c / (2 \alpha^2)$. \mf{replace this figure with the other plot}
% \label{fig:suppFigNegTest} }
% \end{figure}


%\begin{equation}
%    \ket{\Phi_{\pm}(t_C)} \simeq e^{\mp i \pi \alpha^2 /2} \ket{\mp i \alpha} \;, 
%\end{equation}
%which are coherent states with opposite amplitudes, $\ket{\mp i \alpha}$.\\
%Writing Equation (\ref{eq:supp_catTimeState}) with the qubit state in the $\ket{\pm}$ basis, 
%\begin{align}
%\ket{\psi(t=t_\mr{cat})}&\simeq \left( \frac{1+i}{2}\ket{+} + \frac{1-i}{2}\ket{-}\right) \left( c_+\sum_n c_n e^{- igt\sqrt{n}} \ket{n} + c_-\sum_n c_n e^{ igt\sqrt{n}} \ket{n} \right)\\
%&=\ket{-y} \left( c_+\ket{\Phi_+(t)} + %c_-\ket{\Phi_-(t)} \right) \;,
%\end{align}
%makes it clear how at $t=t_\mr{cat}$ the initial combined state of qubit and phonon evolves into a separable state with the qubit in $\ket{-y}$ and the phonon in a superposition of \ket{\Phi_{\pm}(t)} with relative complex amplitudes of that superposition equal to $c_\pm$. Thus, the initial qubit state maps onto the state of the phonon and we observe rotated approximate coherent states for the qubit starting in $\ket{\pm}$ as well as superpositions of said coherent states for the qubit starting in superpositions of $\ket{\pm}$, such as $\ket{\pm y}$ or $\ket{\pm z}$. 
%Choosing $c_+=1/\sqrt{2}$ and $c_-=e^{i\vartheta}/\sqrt{2}$, we retrieve the well-known expression for a Schrödinger's cat state
%\begin{equation}
%    \ket{\psi_\mr{phonon}(t_\mr{cat})}=c_+\ket{\Phi_+(t)} + c_-\ket{\Phi_-(t)} = (\ket{- i \alpha} + e^{i\vartheta} \ket{i \alpha})/\sqrt{2}\;.
%\end{equation}


%For $t\approx t_C$, we can consider again the appoximation $g t \sqrt{n+1} \simeq g t \sqrt{n} + \pi/2$ used in Eq.~\eqref{eq:supp_catTimeState}, and obtain 
%In particular, for $t_C = \pi \alpha/g$ we obtain from Eq.~\eqref{eq:sup_PhiApproxSqrt} that $\ket{\Phi_{\pm}(t_C)} \simeq e^{\mp i \pi \alpha^2 /2} \ket{\mp i \alpha}$. Using this result, and the fact that the system evolution for any qubit initial state $\ket{\psi_q} = (c_+ \ket{+} + c_- \ket{-})$ can be computed using Eq.~\eqref{eq:sup_pmXevol}, we obtain (cfr. Eq.~\eqref{eq:supp_catTimeState} with $c_n\approx c_{n-1}$)
%\begin{equation}
%    U_\mr{JC}(t_{\textit{collapse}})\ket{\psi_q}\ket{\alpha} \simeq \dfrac{1}{\sqrt{2}}\left(\ket{g}-i\ket{e}\right) \left( c_+ e^{-i \pi \alpha^2/2} \ket{-i \alpha} - c_- e^{i \pi \alpha^2/2} \ket{i \alpha} \right) \;.
%\end{equation}




%\subsubsection{moving of the coherent state in the evolution}
%If the qubit is initialized in the state $\frac{1}{\sqrt{2}}(\ket{0}+\ket{1})$, then $c_g=c_e=\frac{1}{\sqrt{2}}$. Then based on Eq.\eqref{eq:sup_exactState}, we can get 

%{\small
%\begin{align}
%    \ket{\Psi(t)} 
%    &= \frac{1}{\sqrt{2}}\sum_{n=0}^\infty \left[ (c_n \cos(g\sqrt{n} t) - i c_{n-1}\sin(g \sqrt{n} t) ) \ket{g} + (c_n\cos(g\sqrt{n+1} t) - i c_{n+1}\sin(g\sqrt{n+1} t) ) \ket{e}
%    \right] \ket{n} \;.\label{eq:init_qubit_x}
%\end{align}
%}
%At here, we define $\Phi_n=g\sqrt{n}t$, and $c_{ng}'(t)=c_n(cos(\Phi_n)-isin(\phi_n)\frac{\sqrt{n}}{\alpha})$, $c_{ne}'(t)=c_n(cos(\Phi_{n+1})-isin(\phi_{n+1})\frac{\alpha}{\sqrt{n+1}})$. Replace these in Eq.\eqref{eq:init_qubit_x}, we can have
%{\small
%\begin{align}
%    \ket{\Psi(t)} 
%    &= \frac{1}{\sqrt{2}}\sum_{n=0}^\infty \left[  c_{ng}'(t)\ket{g} +  c_{ne}'(t)\ket{e}
%    \right] \ket{n} \;.\label{eq:init_qubit_x}
%\end{align}
%}
%Because phonon population of a coherent state has a Poissonian distribution, the standard deviation of $\sigma(1-\frac{\sqrt{n}}{\sqrt{\Bar{n}}})$ is on the order of $O(\frac{1}{\alpha})$, which is a small value when $\alpha$ is big. So we made the approximation that $\frac{\sqrt{n}}{\alpha}=1 $ at here. Based on the Euler formula, we can derive to
%{\small
%\begin{align}
%    c_{ng}'
%    &=c_ne^{-i \Phi _n}\\
%    c_{eg}'&=c_ne^{-i \Phi _{n+1}}\;.
%\end{align}
%}
%If we compare the ratio of the neighbour coefficient
%{\small
%\begin{align}
%    \frac{c_{ng}'(t)}{c_{(n-1)g}'(t)}&=\frac{c_n}{c_{n-1}}e^{-i(\Phi_n-\Phi_{n-1})}\\
%    &=\frac{c_n}{c_{n-1}}e^{-igt(\sqrt{n}-\sqrt{n-1})}\\
%    &=\frac{c_n}{c_{n-1}}e^{-igt\sqrt{n}(1-\sqrt{\frac{n-1}{n})}}\\&\approx \frac{c_n}{c_{n-1}}e^{\frac{-igt}{2\alpha}}\;. \\
%\end{align}

%}
%For the same reason, we can also get 
%\small{
%\begin{align}
%    \frac{c_{ne}'(t)}{c_{(n-1)e}'(t)} \approx \frac{c_n}{c_{n-1}}e^{\frac{-igt}{2\alpha}}\;.
%\end{align}
%}
%The phase $e^{\frac{-igt}{2\alpha}}$ can be interpreted as a rotation of the coherent state, with the angular speed $\frac{-g}{2\alpha}$. If the approximation works perfectly, we would see coherent state rotate in the phase space with the speed $\frac{-g}{2\alpha}$, but because of the approximation, we will see a 'bananaa state' rotation instead. 






==> commented_text.tex <==
% The absurd conclusion of this hypothetical scenario seems to indicate that our current understanding of quantum mechanics is incomplete.

%The bottom chip holds the single junction aluminum qubit which we design for operation in the transmon regime \mb{citation}. The sapphire top chip is used as the HBAR substrate. Coupling between qubit and HBAR is induced through a dome shaped layer of piezoelectric Aluminum Nitride. The piezoelectric acts as a transducer between the electric field of the qubit and the strain field of the HBAR, while the dome shape functions as a curved phononic mirror, confining the phononic mode volume in transverse direction. The phonon modes hosted by this resonator geometry are characterized by two transversal mode numbers $p,l$ and one longitudinal mode number $m$, where the transverse modes are described by Laguerre-Gaussian basis functions and longitudinal modes by sinusoidals respectively. We add a circular antenna below the piezoelectric transducer to shape the transverse qubit electric field into a Gaussian, optimizing for coupling to the fundamental transverse mode with $p=l=0$. 

%With a qubit frequency of around $6\,$GHz, the longitudinal mode we select has a high overtone $m\approx 450$.
%Operating the device in a commercial dilution refrigerator at temperatures around $10\,$mK, the phonon mode we select is operated in the ground state. We then induce resonant energy exchange between qubit and phonon mode by tuning the qubit on resonance for a suitable amount of time. 

%### OLD VERSION: If we consider a coherent state in the acoustic mode, we  find a direct correspondence between the amplitude $\alpha$ of the displaced vacuum state in phase space and the physical oscillation amplitude in longitudinal direction of the atoms in the HBAR mode volume, proportional to $\alpha$ (see supplementary \ref{si:effective mass}). A sketch of the lattice displacement can be seen in the inset of Fig.~\ref{fig1}a). Here the pink and blue atom cores illustrate a crosscut of two neighboring atomic crystal layers, showing a snapshot in time of two longitudinal displacements of opposite amplitudes.

% Continue with half revival time here.
% Considering the time evolution of the full system state without tracing out the phonon subsystem, if the qubit initialized to $\ket{e}$ state, the resonance interaction lead to entanglement between the qubit and phonon state at $t_{\textit{collapse}}$. As a measure for entanglement between qubit and phonon state, we can regard the qubit purity defined as  $\gamma(t)=\text{Tr}\left(\rho_\text{qb}(t)^2\right)$, where $\rho_\text{qb}(t)$ is the reduced density matrix of the qubit subsystem. Monitoring $\gamma(t)$, directly indicates the degree of entanglement in the system during the resonant interaction. Following the trajectory of $\gamma(t)$ in Fig.\ref{fig1}b, the dephasing of Rabi-oscillations coincides with a minimum at $t_{\textit{collapse}}$, indicating a maximally entangled state. 

% Going back to the language of superpositions between out of phase lattice oscillations in the HBAR substrate, we can assign a maximal spatial separation between atoms being part of the created Schr\"odinger's cat state.


% Numerical values for the effective displacements can be found in \ref{si:effective mass}. 
%We can therefor confirm the creation of a coherent superposition between two atomic oscillation states which show a maximal physical distance of $2x^{\text{rms}}_\text{eff}= XXX$ with an effective oscillating mass of $XXX$. 

%As described in previous works\cite{vonLupke22}, our system consists of a plano-convex HBAR fabricated using piezoelectric aluminum nitride (AlN) on a sapphire substrate and a superconducting qubit on a separate sapphire chip, which are then combined into a device called the $\hbar$BAR. The AlN couples the electric field of the qubit with the strain field of the HBAR modes, resulting in a Jaynes-Cummings (JC) type interaction between the two quantum systems.
%Here, we use a single-junction, non-flux tunable transmon qubit and house the $\hbar$BAR inside a superconducting Al cavity. previous devices. All frequency tuning is performed by applying microwave drives to Stark shift the qubit instead of applying an external magnetic field\cite{ChuScience2017}. With our current system parameters and electronic hardware, we are able to Stark shift qubit frequency more than 50 MHz, which enables us to manipulate multiple phonon modes. 
%In order to prepare a cat state of phonons, we make use of the coherent resonant interaction between the acoustic mode and the qubit \cite{BuzekPRA92}. The latter provides the nonlinearity necessary for the preparation of non-Gaussian states of the oscillator. 

%%%%%%%%%%%  Below: Previously Matteo's description of Fig2. Now merged %%%%%%%%%%%         into Fig.1b) explanation. Here we want to discuss 
%%%%%%%%%%%         the experiment only
%For a qubit initially in the excited state, and an phonon mode in the vacuum state, Eq.~\eqref{eq:HJC} results in vacuum Rabi oscillations between the qubit and phonon population~\cite{Chu2018}.
%On the other hand, if the phonon mode is in a coherent state $\ket{\alpha}$, the time evolution of the resonant interaction is considerably more complex \cite{Cummings65,EberlyPRL80}. In particular, it is known that the qubit population oscillates showing periodic collapse and revivals. Intuitively, the collapse occurs because the JC interaction's frequency depends on the number of excitations in the bosonic mode, which for a coherent state is given by a Poissonian distribution. %This oscillation undergoes a collapse due to the dispersion of the Rabi frequencies associated to different photon numbers.
%Therefore, oscillations with different frequencies rapidly dephase, showing a decay of the qubit oscillation amplitude as \cite{Rempe87} $\text{exp}(-(t/t_{\textit{collapse}})^2)$, where $t_{\textit{collapse}}=\sqrt{2}/g$ is the collapse time.
%If the phonon field were classical, the distribution of oscillation frequencies would just result in a decaying signal. However, the phonon energy quantization results in a discrete oscillation frequency spectrum, resulting in oscillations that rephase in finite time. For $\alpha \gg 1$ this revival occurs at $t_R = 2 \pi \alpha/g$ \cite{EberlyPRL80}.

%%%%%%%%%% Matteo's version of Fig2
%Fig.~\ref{fig2}a shows the experimental sequence we use to observe such collapse and revival in our system. First, we prepare the phonon mode in a coherent state by sending a resonant drive pulse of amplitude $A$. After the phonon drive, we cool down the qubit with an ancilla phonon mode to eliminate the effect of the phonon drive on the qubit. Then, we initialize the qubit state in the excited state with a Gaussian shaped $\pi$ pulse. Afterwards, we let then the two system resonantly interact for a time $t$, after which the qubit state is measured. The results are shown in Fig.~\ref{fig2}b for $A=0.35$ (corresponding to $\alpha = 1.75$). As expected, we observe a collapse of the ocillation amplitude after a time $t_{\textit{collapse}}\approx\unit{...}{\mu s}$, and a revival at $t_R\approx\unit{...}{\mu s}$. These effects are genuine quantum features, originating from the phonon energy quantization.
%The observation of revivals in the oscillation also reveals a coherent energy exchange in the qubit-phonon system \cite{MeunierPRL05}. Moreover, it is predicted that at time $t_R/2$ the state of the system resembles a Schr\"odinger's cat state\cite{BuzekPRA92}.

%The first row in Fig.~\ref{fig2}c shows snapshots of the collapse-revival dynamics, obtained by performing Wigner tomography of the phonon mode at different evolution times, using the tools demonstrated in Ref.~\cite{vonLupke22}.
%Here, we normalize the measured Wigner value based on the dispersive parity measurement result of phonon Fock $\ket{0}$ state.
%We normalize the axes of the Wigner functions by measuring the phonon Fock state distribution of coherent states created with different drive amplitudes as demonstrated for example in \cite{Chu2018}. 
%As expected, the initial coherent state (Fig.~\ref{fig2}c upper left), evolves into a cat state at $t_C=2.9\,{\mu s}$ (Fig.~\ref{fig2}c upper middle), and then refocuses into a state that for large $\alpha$ resembles a coherent state ( Fig.~\ref{fig2}c upper right). For comparison, we plot in the second row of Fig.~\ref{fig2}c the exact state evolution we expect from $H_{JC}$  for the interaction time as the corresponding measurement ones (see supp), showing good agreement with the data. 

% Following the linear dependence between $t_R/2$ and $\alpha$, for the measured phonon states displayed in the top row of Fig.~\ref{fig3}a), the smaller initial $\alpha$ result in interaction times $t_C = 2.40\,\mu$s and $2.70\,\mu$s. 

% , as well as a finite background offset of the parity values \cite{vonLupke22}.

%%The extracted state sizes $D$ of the ideal fits, the state sizes $\alpha_\text{fit}$ from the anlytical fits together with the associated fidelities to the reconstructed states are summarized in Fig.\ref{fig3}b. Noting that the interaction times $t_C$ for $A=0.25$ and $A=0.30$ are closer to $t_R/2= 2.42\,\mu$s and $2.90\,\mu$s, when compared to the deviation between $t_C$ and $t_R/2$ for the state with $A=0.35$, we can explain the similar values of $D$ and $\alpha_\text{fit}$ in case of $A=0.25$ and $A=0.30$. Since for these two states, the coherent components are more symmetric around the fringes when compared to the $A=0.35$ state from Fig.\ref{fig2}c, hence fitting to the ideal state gives a larger separation between the coherent state components $\alpha_1$ and $\alpha_2$. Again we accommodate the overall lower fidelities of the ideal states, to the analytical expression \eqref{eq:sup_exactState} only resembling and ideal Schr\"odinger's cat state in the limit $\alpha\rightarrow\infty$ (compare Supplementary A).


% The phase of a cat state is given by the parameter $\vartheta$ in eq.\eqref{eq: ideal_cat}. In the case of $\alpha_1 = -\alpha_2$, $\vartheta = 0$ ($\pi$) corresponds to an even (odd) parity state. 
% % Controlling the phase of the created Schr\"odinger's cat state allows to encode a qubit state in either the even or odd parity subspaces of the bosonic mode's Hilbertspace, a promising method in bosonic error correction codes\cite{Ofek2016}. Considering the Wigner function of Schr\"odinger's cat states, the fringes roll when changing $\vartheta$, where different superposition state shows different interference pattern.  
% To also obtain phase control over the cat states in our system, we vary the initial qubit state across the six cardinal points ($\ket{\pm X}, \ket{\pm Y}, \ket{\pm Z}$ of the Bloch sphere. 
% Since qubit operations are performed far detuned from the selected phonon mode, the qubit state acquires a relative phase in the phonon rotating frame. This results in a phase offset for the rotation axis of the qubit pulse required to reach the cardinal points listed above.
% %We compensate this phase offset by measuring collapse and revivals with the qubit initially prepared in a superposition $\ket{+Z}+e^{i\varphi}\ket{-Z}$, sweeping the phase of the rotation axis $\varphi$. We then pick the phase offset corresponding to the $\ket{+X}$ state, by selecting the one $\varphi$ that does not show oscillations of the qubit population (see supplementary Fig.\ref{fig:suppFig_cnr}). 
% After calibrating the phase offset (see supplementary \ref{Sup A.1}), we perform Wigner tomography on the phonon state with $A=0.30$ at $t_C=2.70\,\mu$s and the qubit initially in $\ket{\pm X}$, resulting in the first column of Fig.\ref{fig3}c. We observe a distorted coherent state located on the upper (lower) half of phase space for the qubit initially in $\ket{+X}$ ($\ket{-X}$), where the separation in phase space is expected from the opposite rotation direction between the two initial qubit states (compare Fig.\ref{fig1}c). As explained earlier, an initial qubit state $\ket{\pm X}$ approximately results in an eigenstate of \eqref{eq:HJC}. We can attribute the state distortions to a finite degree of entanglement during the resonant interaction. 

% Moving to the cardinal points $\ket{\pm Y}=\ket{Z}\pm i\ket{-Z}$, the second column in Fig.\ref{fig3}c shows Schr\"odinger's cat states with opposite phase at $t_C$, revealed by the interference fringes flipping sign between $\ket{+Y}$ and $\ket{-Y}$. We deduce that the phase information of the qubit initial state has fully mapped onto the phonon state at $t_C$. Measurements for the final two cardinal points $\ket{\pm Z}$ are shown in the third column of Fig.\ref{fig3}c. The different shapes between the $\ket{\pm Z}$ states can be understood by noting that for $\ket{+Z}$ the qubit initially is in its ground state, whereas for $\ket{-Z}$ it is prepared in the excited state, contributing one energy quantum $\hbar\omega_{\text{ph}}$ to the total energy of the system when on resonance with the phonon mode. With an average population of $\alpha^2\approx2.3$ of the initial coherent state, the energy contribution of the qubit to the total energy in the system is considerable, leading to the less pronounced fringes. Still the same flipping of parity in the fringes as also observed between $\ket{\pm Z}$ are clearly visible, indicating the qubit rotation angle has mapped onto the phonon state phase at $t_C$.   

% In summary, we conclude the possibility of preparing states that have a fidelity $\geq 65\%$ compared to ideal Schr\"odinger's cat states, with an $\alpha_{\text{fit}}=1.51$, as well as full phase control over the created states by choosing the appropriate initial qubit state.


%%%% Uwe's version
%After showing how we create an approximate cat state in a phonon mode, we move on to demonstrate how we control the amplitude and the phase of such a state. 
%We vary the amplitude $A$ of the initial phonon displacement drive (see Figure \ref{fig2}a) to change the amplitude of the coherent state thus created. 
%As depicted in Figure \ref{fig2} the coherent state evolves into an approximate cat state during an interaction time $t_\mr{cat}\approx t_R/2=\pi\alpha/g$. 
%Note that this time depends on the size $\alpha$ of the coherent state so it has to be adjusted for different cat sizes. 
%The cat state now has an amplitude $\alpha_\mr{cat}$ proportional to the initial drive amplitude $A$. 

%In addition to the cat state depicted in Figure \ref{fig2}c, we show two more cat states with displacement drive amplitudes $A=0.25$ and $A=0.30$ in Figure \ref{fig3}a. 
%As in Figure \ref{fig2}c, we fit the analytical states resulting from a decay-free evolution of the initial coherent state to the data. 
% From the fit we extract the cat sizes $\alpha_\mr{fit}$, displayed in the corner of the Wigner functions of the analytical states in Figure \ref{fig3}a.  
% We also fit an ideal cat state $\ket{\psi_\mr{ideal}}=\ket{\alpha_1}+e^{i\vartheta}\ket{\alpha_2}$ and find the resulting ideal cat size $\alpha_\mr{ideal}=|\alpha_1-\alpha_2|/2$ of the ideal cat state with the highest fidelity to the measured states. 
% We display both the sizes of the best-fit approximate \textcolor{red}{analytical?} and ideal cat states in Figure \ref{fig3}b over the amplitude $A$ of the displacement drive used to create them. 
% We observe a linear relationship between the displacement amplitude and the cat size up to $\alpha_\mr{fit}=1.61$ with fidelities between the density matrix reconstructed from the data and the analytical state around 80\%, as well as fidelities of 65\% and more between the created states and ideal cat states. 

% Now that we have shown how we control the size of the approximate cat states we create, we move to explain how we can control their phase. 
% In an ideal cat state this phase corresponds to the parameter $\vartheta$ in $\ket{\psi_\mr{ideal}}$. 
% In the state created by the evolution under a resonant Jaynes-Cummings interaction between a coherent state in the phonon mode and the qubit, the initial qubit state maps onto the phonon state at the time $t_{cat}$ as follows. 
% Writing the initial qubit state as $\ket{\psi_\mr{qb}(0)} = c_+\ket{+x}+c_{-}e^{i\vartheta}\ket{-x}$, with $\ket{\pm x}=(\ket{g}\pm\ket{e})/\sqrt(2)$, the phase $\vartheta$ is the angle between the complex amplitudes of the $\ket{\pm x}$ states. 
% Over the time $t=t_\mr{cat}$ the phonon state then evolves into a superposition $\ket{\psi_\mr{JC}(t_\mr{cat}}=c_+\ket{\psi_{+}}+c_{-}e^{i\vartheta}\ket{\psi_{-}}$ of two approximately coherent states $\ket{\psi_{\pm}}$. 
% For the detailed derivation, see the Supplementary Information, section \ref{si:state_evolution}. 
% The phase $\vartheta$ and the amplitudes $c_{\pm}$ of this superposition are those of the initial qubit state. 
% In Figure \ref{fig3}c, we show Wigner functions of $\ket{\psi_\mr{JC}(t_\mr{cat})}$ for different initial qubit states, indicated by the label in the top right corner of each plot. 
% When the qubit starts out in $\ket{\pm x}$ (Figure \ref{fig3}c, we observe two misshapen, elongated coherent states, sometimes colloquially referred to as \textit{bananas}. 
% As explained in the Supplementary Information, these states $\ket{\psi_{\pm}}$ approximate displaced coherent states with opposite amplitudes for sufficiently large initial displacements $\alpha$ of the phonon mode. 
% When the qubit starts out in an equal superposition of $\ket{\pm x}$, such as $\ket{\pm y}$ (Figure \ref{fig3}d) or $\ket{\pm z}$ (Figure \ref{fig3}e), the phonon state at $t_\mr{cat}$ is the superposition of the two bananas measured for $\ket{\pm x}$. 
% The position of the fringes is ideally determined by the phase of $\ket{\psi_\mr{qb}(0)}$, which can we observe in Figure \ref{fig3}d and e, noting that the position of the phases for $\ket{\pm y}$ and $\ket{\pm z}$ switches between blue and red. 
% Due to the finite average phonon number $\bar{n}$ in the coherent state the position of the fringes in our experiment differs slightly from the theoretical value corresponding to a $\pi/2$ phase difference between $\ket{\pm y}$ and $\ket{\pm z}$ . 
% The average phonon number for a displacement amplitude of $A=0.35$ is between two and three. Therefore, the energy difference between $\ket{\pm y}$ and $\ket{\pm z}$ changes the effective $\alpha_\mr{fit}$ and in consequence the correct $t_\mr{cat}$. 
% A changing $t_\mr{cat}$ leads to a roll-off of the measured $\vartheta$, because of the detuning between the rotating frame of the qubit drive (which is at the frequency of the qubit rest point) and that of the
% phonon mode. 

% \vspace{10mm}
% \textcolor{blue}{Matteo's version:\\}
% In the following, we demonstrate the control over amplitude and phase of the cat states we can prepare. To generate cat states with different mean phonon number we change the driving pulse amplitude $A$, and adjust the resonant evolution time accordingly. 
% In order to benchmark the generated cat states, we implement a maximum-likelihood reconstruction of the system's state $\rho$ from the collected parity measurements \cite{Chou2018}, and then compute the fidelity against a target state $\sigma$ as $F=\text{Tr}\left[\sqrt{\sqrt{\rho}\sigma\sqrt{\rho}}\right]$. As a first target state, we consider the analytical state resulting from evolving a coherent state $\alpha_a$ according to $H_{JC}$, see Supp Info. As a second target state, we consider the ideal cat state $\Psi_1 = \ket{\alpha_1} + e^{i\vartheta} \ket{\alpha_2}$, having amplitude $\alpha_i=\vert\alpha_1-\alpha_2\vert^2/2$. \mf{Maybe different name for the size? Like Haroche's $D$?}

% In Fig.\ref{fig3}a we show the measured Wigner functions of cat states prepared with two different values for $A$, together with the best matching analytical state resulting from evolving a coherent state $\ket{\alpha_1}$ with $H_{JC}$. These amplitudes $\alpha_1$, together with the amplitudes $\alpha_2$ of the best matching ideal cat states and with the associated fidelities, are summarized in Fig.\ref{fig3}b. We conclude the possibility of preparing states that have a fidelity $\geq 65\%$ compared to ideal cat states.

% Apart from the amplitude, it is of interest to control also the phase of the cat state, which is associated to the position and parity of the Wigner's interference fringes. In the limit of large $\alpha$ this phase can be fully controlled by the phase of the initial qubit state. In fact, one can observe collapse-revival dynamics for any initial qubit state on the $yz$-plane, resulting at $t_C$ in cat states with different phases (cite supp). On the other hand, preparing the initial qubit state along the $\pm x$ direction does not give any evolution to the oscillator's coherent state, as these are quasi-eigenstates of $H_{JC}$ \cite{GeaPRL90}.

% We demonstrate these ideas experimentally, by initializing the qubit's state along direction $\vec{v}\in\{\pm x, \pm y, \pm z \}$ before letting it interact resonantly for a time $t=...$ with the phonon mode prepared with $A=0.035$. The results are shown in Fig.\ref{fig3}c, where we can see the phonon mode to stay similar to a coherent state for $\vec{v} = \pm x$, while it evolves to cat states with different phases for $\vec{v} = \pm y,\pm z$. This measurement gives also an intuitive understanding of the dynamics resulting into cat states: an arbitrary qubit state can be seen as a superposition of $x$ eigenstates, and thus the evolution of the field as a superposition of evolutions of counter-rotating coherent states.

% \mf{Mention that the ability of preparing cat states with arbitrary phase is of interest for bosonic encoding of quantum information [Kerr cat qubit, ..].}



On the other hand, a coherent state should have a characteristic decay time $2T_1^{\text{ph}}$ to vacuum.



In the top row of Fig.~\ref{fig4}a, we show snapshots of the largest cat state with $A=0.35$ and $\alpha_\text{fit}=1.61$ at three different wait times $\tau=1, 5,$ and $50\,\mu$s, together with the reconstructed states in the row below. Note the fast decay of negative parity values after $5\,\mu$s compared to the slower decay speed of the classical state components towards the vacuum state. To quantify the characteristic timescale for the disappearance of quantum features, we make use of the time dependent negativity defined as $\delta(t) \equiv \int d^2\beta\,\vert W(\beta,\alpha, t)\vert - W(\beta,\alpha, t)$. Here, $W(\beta,\alpha, t)$ is the Wigner function of the cat state of size $\alpha$ at time $t$, and the integration is over all phase space, parametrized by the complex displacement amplitude $\beta$. Since $\delta(t)$ represents an integration over all negative values of $W(\beta, \alpha, t)$, it can be considered a measure for non-classicality of the state\cite{Kenfack04}. As shown in supplementary \ref{si:cat_decoherence}, in the limit of large $\alpha$,  $\delta(\tau)$ decays with a time constant $\tau_\text{cat}=T_1^{\text{ph}}/(2\alpha^2)$, while a coherent state should have a characteristic decay time $2T_1^{\text{ph}}$ to vacuum, explaining the different decay times of the aforementioned features in Fig.\ref{fig4}a.


We experimentally extract the timescales of negativity decay for cat states with four different initial displacement amplitudes $A$. Due to fluctuations of the qubit frequency during the dispersive interaction, we observe fluctuations in the background value of the measured Wigner functions \cite{vonLupke22}. We mitigate the contribution of these variations to the computed negativity by manually selecting an integration window in phase space enclosing only the interference fringes in the reconstructed state, where negative features of the Wigner function are expected to appear. We then calculated the negativity within this window using the measured Wigner function, which are together with the corresponding fits to an exponential decay model are presented in Fig.\ref{fig4}b.  The fitted negativity decay constants for all four cat state sizes are shown in Fig.\ref{fig4}c.
Apart from the smallest state size, we observe the decay times monotonically decreasing with $A$. This trend is confirmed by looking at the extracted decay times obtained from a full Master equation simulation of the state decay with the reconstructions of the measured states set as the intial state in the simulation. An explanation for the low decay time of the smallest cat state is given in supplementary Fig.\ref{fig:suppFigCatPhaseDecays}. Simulating the decay of an ideal Schr\"odinger cat state (see eq.\eqref{eq: ideal_cat} with different $\vartheta$ and $\alpha_1 =-\alpha_2$, it can be seen that for state sizes $\alpha_1\lesssim1.5$, the decay rate becomes dependent on $\vartheta$. For $\vartheta$ small, this results in a drop in the decay time below $\alpha_1\lesssim 1.1$ coinciding with the decay time we observe in the reconstructed negativity of the smallest state.    

% \vspace{10mm}
% \textcolor{blue}{Matteo's version:\\}
% Superposition states are non-classical states that are notoriously prone to dec
herence. In order to investigate the quantum to classical transition of such states, we let the states we prepare evolve freely for some time $t$ before performing Wigner tomography. Then, we compute the negativity of the reconstructed Wigner function at time $t$ as $\delta(t) \equiv \int d^2\alpha \Big( \vert W(\alpha)\vert - W(\alpha) \Big)$, which is an indicator of nonclassicality~\cite{Kenfack04}. Computing the negativity at different times allows us to observe the disappearence of quantum coherences, and to extract the associated timescale.

% In Fig.~\ref{fig4}a we show a selection of snapshots for the decay of a cat state prepared with $A=XXX$. Similar measurements have been taken for the cat states with $A=XXX$. Selecting a phase-space region enclosing the fringes we are able to compute reliably $\delta(t)$, without being much affected by noise and imperfections in the background. The values we obtain are shown in Fig.~\ref{fig4}b, together with an exponential fit of the data. The decaying rates thus obtained are summarized in Fig.~\ref{fig4}c, together with theoretical and simulated predictions. 


% [drafted:] In Ref.~\cite{BrunePRA92,DelegliseNat08} it was investigated the decoherence of photon cat states under cavity losses at rate ($1/T_1$). It was found both theoretically and experimentally that off-diagonal elements decay for small times as $T_1/(2 \alpha^2)$ \mf{Here it would be beneficial to use a cat size parameter, rather than alpha.} We note that the same decay time is observed for the negativity of cat states of size $\alpha\gtrsim 2$ (see Supp Info). As our states are smaller than this, we perform a numerical simulation to predict their lifetime. The results are shown in Fig.~\eqref{fig4}c, and show good agreement between theory and simulation. 



% We measured Wigner functions of the generated cat state by the dispersive phonon parity measurement technique. The largest size of the generated cat state is $\alpha=1.51$, with a measured fidelity of $F\approx65\%$. We investigated the phase of generated cat state by initializing the qubit with different phase in the cat state generation sequence. 


% Generation the superposition of coherent states in macroscopic mechanical system is not only interesting in investigating the fundamental physics, such as collapse model of the macroscopic objects and the boundary between the classic and the quantum, but also useful ingredients for quantum information processing, such as quantum error correction and quantum metrology. For example, cat state in bosonic coding has been proposed and generated in cQED system, and $\hbar$BAR systems even have extra advantage of doing this, since the FSR of $\hbar$BARs is small and more phonon modes are available. In combination of the dispersive measurement of the phonon parity, error correction can be implemented in the cat state. Cat state has also been proposed for quantum metrology due to the high Fisher information at the fringe region. As a mechanical system, $\hbar$BAR can also be used for quantum-enhanced frequency or force sensing. For both investigating the fundamental physics and quantum information processing, requirements on qubit phonon coupling strength and sample coherence are similar, which implies better fabrication technique and device design is needed.


% We performed the Wigner tomography of these phonon states by using the displaced parity measurement procedure described in [parity paper]. 


% Each reconstructed phonon state $\rho_{r}$ was optimized for with Maximum Likelihood Estimation (MLE) fits to these measured Wigner functions, as described in Schoelkopf 2018: By imposing non-negative eigenvalues, Hermiticity and unit trace, we constrain the fit to only physical density matrices $\rho$. Each measured Wigner function is a set of measurement outcomes. Every $\rho$ will have an expectation value corresponding to each of these outcome. To find the MLE state $\rho_r$, we minimize the residual sum of squares over all measurements. The resulting optimization is a convex problem that can be efficiently solved as a constrained semi-definite programming problem.
% (Section S6B of https://arxiv.org/pdf/1801.05283.pdf)

% \textcolor{magenta}{Here we need to talk about the rescaling. For the reconstruction we can just cite previous work.} 

% Experimental imperfections and noise can give the measured Wigner functions artificially-offset features in the background. Simply carrying out the integral in Eq.~\eqref{eq:supp_WNegDef} over the full Wigner function phase space would therefore give an additionally noisy negativity estimate. To account for this background problem, we limit the integral to a sub-region of the phase space--the smallest sized window that fully encloses the negative fringes of each cat state. Using this method, we do not include any unphysical negative features present in the Wigner function, outside of the cat state, in our analysis of the negativity decay. Since we specify the windows to fully enclose all negative fringes of the cat state, performing the integral in Eq.~\eqref{eq:supp_WNegDef} only over the sub-region gives the same result as integrating over the full region (in the case of an ideal cat state with a perfect background). 

% To simulate the negativity decay of these states...


% \begin{figure}
% \centering
% \includegraphics[width=10cm]{figures/suppFigNegTest.pdf}
% \caption{\textbf{Cat decoherence rate from negativity.}
% Comparison between the cat decoherence rate obtained from a numerical computation of the Wigner negativity decay rate, and the rate $\tau_\text{cat} = T_c / (2 \alpha^2)$. \mf{replace this figure with the other plot}
% \label{fig:suppFigNegTest} }
% \end{figure}


%\begin{equation}
%    \ket{\Phi_{\pm}(t_C)} \simeq e^{\mp i \pi \alpha^2 /2} \ket{\mp i \alpha} \;, 
%\end{equation}
%which are coherent states with opposite amplitudes, $\ket{\mp i \alpha}$.\\
%Writing Equation (\ref{eq:supp_catTimeState}) with the qubit state in the $\ket{\pm}$ basis, 
%\begin{align}
%\ket{\psi(t=t_\mr{cat})}&\simeq \left( \frac{1+i}{2}\ket{+} + \frac{1-i}{2}\ket{-}\right) \left( c_+\sum_n c_n e^{- igt\sqrt{n}} \ket{n} + c_-\sum_n c_n e^{ igt\sqrt{n}} \ket{n} \right)\\
%&=\ket{-y} \left( c_+\ket{\Phi_+(t)} + %c_-\ket{\Phi_-(t)} \right) \;,
%\end{align}
%makes it clear how at $t=t_\mr{cat}$ the initial combined state of qubit and phonon evolves into a separable state with the qubit in $\ket{-y}$ and the phonon in a superposition of \ket{\Phi_{\pm}(t)} with relative complex amplitudes of that superposition equal to $c_\pm$. Thus, the initial qubit state maps onto the state of the phonon and we observe rotated approximate coherent states for the qubit starting in $\ket{\pm}$ as well as superpositions of said coherent states for the qubit starting in superpositions of $\ket{\pm}$, such as $\ket{\pm y}$ or $\ket{\pm z}$. 
%Choosing $c_+=1/\sqrt{2}$ and $c_-=e^{i\vartheta}/\sqrt{2}$, we retrieve the well-known expression for a Schrödinger's cat state
%\begin{equation}
%    \ket{\psi_\mr{phonon}(t_\mr{cat})}=c_+\ket{\Phi_+(t)} + c_-\ket{\Phi_-(t)} = (\ket{- i \alpha} + e^{i\vartheta} \ket{i \alpha})/\sqrt{2}\;.
%\end{equation}


%For $t\approx t_C$, we can consider again the appoximation $g t \sqrt{n+1} \simeq g t \sqrt{n} + \pi/2$ used in Eq.~\eqref{eq:supp_catTimeState}, and obtain 
%In particular, for $t_C = \pi \alpha/g$ we obtain from Eq.~\eqref{eq:sup_PhiApproxSqrt} that $\ket{\Phi_{\pm}(t_C)} \simeq e^{\mp i \pi \alpha^2 /2} \ket{\mp i \alpha}$. Using this result, and the fact that the system evolution for any qubit initial state $\ket{\psi_q} = (c_+ \ket{+} + c_- \ket{-})$ can be computed using Eq.~\eqref{eq:sup_pmXevol}, we obtain (cfr. Eq.~\eqref{eq:supp_catTimeState} with $c_n\approx c_{n-1}$)
%\begin{equation}
%    U_\mr{JC}(t_{\textit{collapse}})\ket{\psi_q}\ket{\alpha} \simeq \dfrac{1}{\sqrt{2}}\left(\ket{g}-i\ket{e}\right) \left( c_+ e^{-i \pi \alpha^2/2} \ket{-i \alpha} - c_- e^{i \pi \alpha^2/2} \ket{i \alpha} \right) \;.
%\end{equation}




%\subsubsection{moving of the coherent state in the evolution}
%If the qubit is initialized in the state $\frac{1}{\sqrt{2}}(\ket{0}+\ket{1})$, then $c_g=c_e=\frac{1}{\sqrt{2}}$. Then based on Eq.\eqref{eq:sup_exactState}, we can get 

%{\small
%\begin{align}
%    \ket{\Psi(t)} 
%    &= \frac{1}{\sqrt{2}}\sum_{n=0}^\infty \left[ (c_n \cos(g\sqrt{n} t) - i c_{n-1}\sin(g \sqrt{n} t) ) \ket{g} + (c_n\cos(g\sqrt{n+1} t) - i c_{n+1}\sin(g\sqrt{n+1} t) ) \ket{e}
%    \right] \ket{n} \;.\label{eq:init_qubit_x}
%\end{align}
%}
%At here, we define $\Phi_n=g\sqrt{n}t$, and $c_{ng}'(t)=c_n(cos(\Phi_n)-isin(\phi_n)\frac{\sqrt{n}}{\alpha})$, $c_{ne}'(t)=c_n(cos(\Phi_{n+1})-isin(\phi_{n+1})\frac{\alpha}{\sqrt{n+1}})$. Replace these in Eq.\eqref{eq:init_qubit_x}, we can have
%{\small
%\begin{align}
%    \ket{\Psi(t)} 
%    &= \frac{1}{\sqrt{2}}\sum_{n=0}^\infty \left[  c_{ng}'(t)\ket{g} +  c_{ne}'(t)\ket{e}
%    \right] \ket{n} \;.\label{eq:init_qubit_x}
%\end{align}
%}
%Because phonon population of a coherent state has a Poissonian distribution, the standard deviation of $\sigma(1-\frac{\sqrt{n}}{\sqrt{\Bar{n}}})$ is on the order of $O(\frac{1}{\alpha})$, which is a small value when $\alpha$ is big. So we made the approximation that $\frac{\sqrt{n}}{\alpha}=1 $ at here. Based on the Euler formula, we can derive to
%{\small
%\begin{align}
%    c_{ng}'
%    &=c_ne^{-i \Phi _n}\\
%    c_{eg}'&=c_ne^{-i \Phi _{n+1}}\;.
%\end{align}
%}
%If we compare the ratio of the neighbour coefficient
%{\small
%\begin{align}
%    \frac{c_{ng}'(t)}{c_{(n-1)g}'(t)}&=\frac{c_n}{c_{n-1}}e^{-i(\Phi_n-\Phi_{n-1})}\\
%    &=\frac{c_n}{c_{n-1}}e^{-igt(\sqrt{n}-\sqrt{n-1})}\\
%    &=\frac{c_n}{c_{n-1}}e^{-igt\sqrt{n}(1-\sqrt{\frac{n-1}{n})}}\\&\approx \frac{c_n}{c_{n-1}}e^{\frac{-igt}{2\alpha}}\;. \\
%\end{align}

%}
%For the same reason, we can also get 
%\small{
%\begin{align}
%    \frac{c_{ne}'(t)}{c_{(n-1)e}'(t)} \approx \frac{c_n}{c_{n-1}}e^{\frac{-igt}{2\alpha}}\;.
%\end{align}
%}
%The phase $e^{\frac{-igt}{2\alpha}}$ can be interpreted as a rotation of the coherent state, with the angular speed $\frac{-g}{2\alpha}$. If the approximation works perfectly, we would see coherent state rotate in the phase space with the speed $\frac{-g}{2\alpha}$, but because of the approximation, we will see a 'bananaa state' rotation instead. 





